Exploring the Tradeoff between Competitive Ratio and Variance in Online-Matching Markets

In this paper, we propose an online-matching-based model to study the assignment problems arising in a wide range of online-matching markets, including online recommendations, ride-hailing platforms, and crowdsourcing markets. It features that each assignment can request a random set of resources and yield a random utility, and the two (cost and utility) can be arbitrarily correlated with each other. We present two linear-programming-based parameterized policies to study the tradeoff between the \emph{competitive ratio} (CR) on the total utilities and the \emph{variance} on the total number of matches (unweighted version). The first one (SAMP) is to sample an edge according to the distribution extracted from the clairvoyant optimal, while the second (ATT) features a time-adaptive attenuation framework that leads to an improvement over the state-of-the-art competitive-ratio result. We also consider the problem under a large-budget assumption and show that SAMP achieves asymptotically optimal performance in terms of competitive ratio.

==> 2-intro.tex <==


\subsection{Preliminaries and Main Contributions}

\xhdr{Competitive ratio}. Competitive ratio (CR) is a commonly-used metric to evaluate the performance of online algorithms. Consider  maximization of the total utilities as studied here for example. 
Let $\ALG(\mathcal{I})=\E_{S \sim \cI} [\ALG(S)]$ denote the expected performance of $\ALG$ on an input $\mathcal{I}$, where the expectation is taken over the 
the random arrival sequence $S$ of  online agents, random outcomes of cost and profit, and 
the random seed in $\ALG$.  
Let $\OPT(\mathcal{I})=\E[\OPT(S)]$ denote the expected performance of an \emph{offline optimal}(denoted by \OPT), where \OPT have the previlege to access to the full arrival sequence of online agents before optimizing its matching decisions.  The competitive ratio is then defined as $\inf_{\mathcal{I}} \frac{\ALG(\mathcal{I})}{\OPT(\mathcal{I})}$. Here are several points for $\OPT$: (1) It can choose an arbitrary order to process online agents instead of being required to strictly follow their arrival order; (2) It can access to the set of all arriving online agents in advance but not the random realizations of cost and profit on each assignment relevant to arriving agents. The latter can be observed only after \OPT decides to make that assignment; (3) It conforms to the  safe-policy requirement as well.  It is a common technique to use an \LP to upper bound the $\OPT(\mathcal{I})$ (called the benchmark \LP) and hence get a valid lower bound on the target competitive ratio. In the following, we give a toy example showing how to compute the competitive ratio in an exact way. 


%Note that (1) \OPT can access to the random realizations of cost and profit on an edge $e$ only after \OPT decides to match $e$. the offline optimal can choose an arbitrary order to process online agents instead of being required to strictly follow their arrival order. 






\begin{example}
Suppose we have a star graph where we have one single offline vertex $i=1$ and two online vertices $j=a,b$. We have $T=2$ rounds and during each round, the arrival distribution is 
$q_a=1/3, q_b=2/3$. In other words, in each round online agents $a$ and $b$ will be sampled (with replacement) with respective probabilities $1/3$ and $2/3$. We have $K=2$ resources and each has a unit budget $B_1=B_2=1$. For the edge $(i=1,j=a)$, with probability $1/2$, $\cA_a=(1,0)$ and $W_a=1$; with another probability $1/2$, $\cA_a=(0,1)$ and $W_a=1$. For the edge $(i=1,j=b)$, with probability $1/2$, $\cA_b=(1,1)$ and $W_b=2$; with another probability $1/2$, $\cA_b=(0,0)$ and $W_b=0$. Observe that on our instance, the sparsity $\Del=2$. In the following, we analyze the performance of Greedy, that is to accept whatever arriving online agent during $t=1$ and $t=2$, if possible. 

Note that the four possible arrival sequences and corresponding probabilities are as follows: $\{(a,a), 1/9\}$, $\{(a,b), 2/9\}$, $\{(b,a), 2/9\}$, and $\{(b,b), 4/9\}$. For $S=(a,a)$, the performance of \gre is $\gre(a,a)=1$. For ease of notation, let $a_1, a_2$ be the two agents arriving at $t=1,2$, respectively. Recall that we consider safe policies only and thus, \gre will stop considering $a_2$ since with a chance of $1/2$, adding $a_2$ might cause an overflow of budget for whatever observed cost realization of $a_1$. Note that the safe-policy rule applies to the offline optimal $\OPT$ as well. Thus, $\OPT(a,a)=1$. For $S=(a,b)$, we have $\gre(S)=1$ since $\gre$ will stop considering $b$ after its arrival. However, $\OPT(S)=3/2$: \OPT will first process $b$ and then $a$. In that case, with probability $1/2$, $\OPT$ gets a value of $2$ and stop, and with another probability $1/2$, $\OPT$ gets a value $0$ and will continue to accept $a$ that leads to another expected value of $1$. Similarly, we can verify that for $S=(b,a)$, $\gre(S)=\OPT(S)=3/2$, and for $S=(b,b)$, $\gre(S)=\OPT(S)=3/2$. In summary, we have the expected performance of \gre is $(1/9) \cdot 1+(2/9)\cdot (1+3/2)+(4/9) \cdot (3/2)=12/9$ and that of $\OPT$ is $(1/9) \cdot 1+(2/9)\cdot (3/2+3/2)+(4/9) \cdot (3/2)=13/9$. This implies that the competitive ratio of \gre is equal to $12/13$ on the toy example.  $\hfill \square$
 \end{example}



\xhdr{Main contributions.} 
Our contributions can be summarized as follows. First, we present a benchmark LP (\LP~\eqref{obj-1}), whose optimal value is shown to be a valid upper bound for the offline optimal. Second, we give two LP-based algorithms. The first one (\adap) incorporates simulation-and-attenuation techniques into the online sampling process, which achieves a nearly optimal online ratio. The second one (\nadap) just applies an online sampling process guided by an optimal solution to the benchmark LP, and we give a \emph{tight}  online competitive analysis under the large-budget assumption. Throughout this paper, we assume \LP~\eqref{obj-1} as the default benchmark LP, and all competitive-ratio results are obtained when taking $T \rightarrow \infty$\footnote{This is a common assumption among literatures studying online-matching models under KIID, see, \eg \citep{haeupler2011online,manshadi2012online,jaillet2013online,brubach2016new}.}.

 
\begin{theorem}\label{thm:main-1}
There exists a simulation-and-attenuation based algorithm ($\adap$), which achieves an online competitive ratio of $\Big(1-\sfe^{-\Del}\Big)/\Del$. Meanwhile, no algorithm can achieve an online competitive ratio better than  $\Big(1-\sfe^{-(\Del-1+1/\Del)}\Big)/(\Del-1+1/\Del)$. Both the lower and upper bounds are with respect to the benchmark \LP~\eqref{obj-1}.
\end{theorem}

\textbf{Remarks}. (1) When $\Del=1$, the lower and upper bounds match with each other and both are equal to $1-1/\sfe$, which suggests the tightness of our online analysis. 
(2) \citet{aamas-19} considered a special case of \mb where each assignment has a \emph{deterministic} vector-valued cost with sparsity $\Del$ but under known adversarial distributions, which allow the arrival distributions to change over online rounds. They gave an upper bound (hardness result) of $1/(\Del-1+1/\Del)$ and a lower bound of $1/(\Del+1)$, respectively.  Note that both of the lower and upper bounds are improved here as shown in Theorem~\ref{thm:main-1} since $(1-\sfe^{-\Del})/\Del \ge \big(1-1/(\Del+1)\big)/\Del=1/(\Del+1)$. One key technical improvement is an attenuation scheme that is adaptive to the arriving time of online agents. In contrast,  \citet{aamas-19} uses a static attenuation scheme that is oblivious to the arriving time of online agents. (3) \citet{brubach2016new} considered a variant of online stochastic matching, which can be cast as a \emph{strict} special case of \mb in the way that each assignment has a Bernoulli random vector-valued cost with $\Del=1$. From Theorem~\ref{thm:main-1},  \adap achieves an online ratio of $1-1/\sfe$ when $\Del=1$, which matches that of~\citep{brubach2016new}. (4)~\citet{kess13} considered online $\Del$-hypergraph matching that can be cast as a special case of our model where each assignment takes a deterministic cost vector with sparsity $\Del$. They considered the random arrival order and gave an online competitive ratio of $1/(\sfe \cdot \Del)$. 



 

% In contrast, [X] gave a simple simulation-based online policy which achieves a ratio of $1/(\Del+1)$ but under KAD. Thus, we improve both upper and lower bounds presented in [XX]. (2) Our ratio is tight when $\Del=1$. Also, our model includes OSM with stochastic rewards under KIID as considered in [ESA 16] as a special case with $\Del=1$. We provide a general analysis and get the same ratio as [ESA 16]. (3) Compare our results to [XX, Will Ma], we do not consider patience constraints imposed on online agents. 
%$\nadap$ with $\gam=\frac{1}{\Del}$ 
%\vspace{0.1in}

%\begin{theorem}\label{thm:main-2}
%There exists a simple LP-based sampling algorithm $\nadap(\gam)$ which achieves a competitive ratio at least  $\frac{1}{2 \Del}$ with $\gam=1/\Del$.
%\end{theorem}


Let $B=\min_k B_k$, which denotes the minimum budget over all resources. When all budgets are large (\ie $B \gg 1$), we offer a simple LP-based sampling algorithm $\nadap$, which has an asymptotically optimal ratio.

   \begin{theorem}\label{thm:main-3}
There exists a simple LP-based sampling algorithm $\nadap$ such that 
(a) it achieves an online competitive ratio of  $1-\frac{1}{\sqrt{2\pi B}}(1+o(1))$ when $\Del=1$; (b) it achieves online competitive ratio of $1- \kappa \cdot  \sqrt{\frac{\ln \Del}{B}}(1+o(1))$ with $\sqrt{2}<\kappa \le 2\sqrt{2}$. The online analysis for both cases (a) and (b) are tight with respect to  the benchmark \LP~\eqref{obj-1}. 
\end{theorem}

% (3) The optimality of online ratios stated here is all with respect to our default benchmark \LP~\eqref{obj-1}.

\textbf{Remarks}. (1) The term $o(1)$ in part (a) vanishes when $B \rightarrow \infty$, while that in part (b) vanishes when $B=\omega(\ln \Del)$ and $\Del \rightarrow \infty$.  (2) As mentioned before,~\citet{brubach2016new} considered a strictly special case of \mb with $\Del=1$. When all budgets are large, they gave an algorithm achieving an asymptotical online ratio of $1-B^{-1/2+\ep}(1+o(1))$ for any given $\ep>0$. Our result in part (a) significantly improves that. (2) The constants of the leading terms as stated in parts (a) and (b) are optimal with respect to our current benchmark \LP~\eqref{obj-1}, which are $\frac{1}{\sqrt{2\pi}}$ and $\kappa$, respectively. That is to say, \eg no online algorithm can achieve an online ratio of $1-\frac{c}{\sqrt{2\pi B}}(1+o(1))$ with a constant $c<1$ when $B \gg 1$ and $\Del=1$ if compared against the optimal value of \LP~\eqref{obj-1}. (3) The result of part (a) in Theorem~\ref{thm:main-3} (\ie $1-\frac{1}{\sqrt{2\pi B}}(1+o(1))$) appears in multiple contexts before such as Adwords and correlation gap~\cite{devanur2012asymptotically,alaei2012online,yan2011mechanism}. However, the analysis and focus here are essentially different from there. Let $\Ber(B/T)$ denote a Bernoulli random variable with mean $B/T$. For Adwords and related applications~\cite{devanur2012asymptotically,alaei2012online,yan2011mechanism}, they all care about $\E[\min(X,B)]/B$ when $T$ is sufficiently large, where $X$ is the sum of $T$ \iid $\Ber(B/T)$s. In contrast, we care about $\E[\min(T',T)]/T$, where $T'$ is the number of copies of  \iid  $\Ber(B/T)$s needed such that the total sum is equal to $B$. Though we can draw a subtle connection between the two (see the proof in Section~\ref{sec:proof-part-a}), it is not straightforward to see the two are the same. 


\section{Other Related Work}

 Our problem falls under the  family of \emph{online packing} problems. There have been a a few recent studies on this. The works of of~\citep{agrawal2014dynamic,agrawal2014fast,buchbinder2009online} all  considered the arrival setting of random arrival order (RAO), which is less restrictive than KIID as considered here. Under RAO, a powerful algorithm-design paradigm  is the primal-and-dual approach, see the survey book~\citep{buchbinder2009design}.
It is interesting to compare the setting studied here with those of~\cite{kess-stoc} and~\cite{jacm19}, both of which considered online resource allocation with multiple budget constraints under RAO. However, they assumed that for each assignment both the cost vector and profit are deterministic. Here we assume each assignment can have a random vector-valued cost and a random reward, and the two can be arbitrarily correlated with each other. Another difference is that they considered fractional cost in the way that each $\cA_e \in [0,1]^K$ (deterministic) while we assume that each $\cA_e \in \{0,1\}^K$ (random) here.~\citet{jacm19} gave an online ratio of $1-\omega(\sqrt{\ln \Del/B})$, which was improved to $1-O(\sqrt{\ln \Del/B})$ by \citet{kess-stoc}. Note that the work of \cite{kess-stoc} has not identified the proper constant included in the term $O(\sqrt{\ln \Del/B})$, whereas it is a main focus of this paper.


The offline version of our problem captures the stochastic $\Del$-set packing problem as a special case, which was introduced by~\citet{bansal2012lp}. They gave a $2\Del$-approximation algorithm for the stochastic $\Del$-set packing problem, which was improved to $\Del+o(\Del)$ by~\citet{TALG-20} later.~\citet{baveja2018improved} considered $\Del$-uniform stochastic hypergraph matching, which can be viewed as a special case of the stochastic $\Del$-set packing problem. They gave two approximation algorithms that achieve a ratio of $\Del+1/2$ and a ratio of $\Del+\ep$ for any given $\ep>0$, respectively.


%\xhdr{Main techniques}. The improvement in the results of Theorem~\ref{thm:main-1} is due to a more carefully designed attenuation scheme as stated in Lemma~\ref{lem:adap} compared with~\cite{aamas-19}. In~\cite{aamas-19}, they tried to make sure each assignment $e=(i,j)$ is successfully scheduled with a probability $\gam \cdot x_e^*$, where $x_e^*$ is an optimal solution to the benchmark LP, and where $\gam$ is a target ratio regardless of when $j$ arrives. In our algorithm \adap, we set $\gam$ as a function of $t$ which is the time when $j$ arrives. The main challenges in the proof Theorem~\ref{thm:main-3} lie in the following parts: (1) How to identify the worst scenario of the algorithm \nadap (\ie the instance on which the worst online competitive ratio is achieved)? (2) How to compute the the lower and upper bound on the ratio achieved by \nadap in the worst scenario? The proof of Theorem~\ref{thm:main-3} is highly technically involved and includes a detailed analysis of a bins-and-balls model as stated in Section~\ref{sec:two-thms}. 



 

%To prove the upper bound, we mainly utilize the property of \emph{negative association} and Slud's Inequality~\citep{slud1977distribution}. For the lower bound, we apply the Lemma 5.10 on page 110 of the book~\citep{mitzenmacher2017probability}.  




%All these results assume no large-budget assumption. Note that under the same assumption (small budgets), we gave an algorithm for \mb which achieves an online competitive ratio of $(1-\sfe^{-\Del})/\Del$ as shown in Theorem~\ref{thm:main-1}. 


%This suggests that for a maximization problem as studied here, online version can be as easy as the offline version. 

% which achieve approximation ratios of $1/(2\Del)$ and $1/(\Del+1)$ for the general case and monotone cases, respectively. The latter refers to the scenario when each item 



%Recently, [Will] considered online assortment optimization problem with inventory constraints. They proposed an online matchi
%Mention that paper of Will. Notice that for general assortment, they assume (a) each round we can show at most $\ell_j$ assortment $S$ from $\cS$ (the set of all feasible assortments in the platform) and $\{0\} \in \cS$; (b) each item has a unit capacity (WLOG by creating multiple copies but not good for large capacities); (c) each user will accept at most one item each round; (d) their results rely on such a key assumption that either $\ell_j \ge |\cS|$ or $\sum_{S \in \cS} \sum_{i \in S} p_j(i,S) \le 1$; (e) an item can be repeated shown to an user within one round if not accepted before. Our model had better stated as a bundle: let $
%\cS_j$ be the set of all feasible bundles relevant to user of type $j$; once shown a bundle $S \in \cS_j$, user $j$ has only two possible choices, either accept it with a certain probability $p_{j,S}$ (\ie accept all items in it instead of a partial set of items of $S$) or reject it otherwise. We assume all user has a unit patience, \ie each user can be shown at most one bundle.  













==> 5-nadap-old.tex <==



  \section{A Simple Sampling Algorithm}
 In this section we present a simple  sampling algforithm, which works well for the case of large budgets.
 \bluee{Perhaps at the beginning of this section check if we state the generalization of setting to fractional}.
 % Let $\gam \in (0,1]$ be a given parameter. 
 %\redd{Perhaps we just present it as $\nadap$ and assume $\gam=1$ by default?} 
 
  
 \begin{algorithm}[h!]
\DontPrintSemicolon
Let an online agent of $j$ arrive at time $t$. \;
Sample an assignment $e \in E_{j}$ with probability $ x^*_e/r_j$. \label{nalg:step3}\;
If $f$ is safe, then make it; otherwise, reject $j$. 
\caption{An LP-based Sampling algorithm: $\nadap$}
\label{alg:nadap}
\end{algorithm}

Observe that Step~\eqref{nalg:step3} of $\nadap(\gam)$ is valid since $\sum_{e \in E_j} \gam \cdot x^*_e/r_j \le \gam  \le 1$ due to Constraint~\eqref{cons:j} in \LP-\eqref{obj-1}. 

 A key lemma to prove Theorem~\ref{thm:main-2} is as follows. 
 Consider a given $t^* \le T$ and an assignment $e^*$. Recall that $\beta_{e^*,t^*}=\Pr[\SF_{e^*,t^*}=1]$ is the probability that $e^*$ is safe at time $t^*$. 
 \vspace{0.1in}
 \begin{lemma}\label{lem:nadap-1}  
 For any given $0<\gam \le 1$, we have $\beta_{e^*,t^*} \ge 1-\gam \Del (t^*-1)/T$. 
\end{lemma}


\begin{proof}
Consider a given $k \in \cS_{e^*}$. Let $U_{k,t^*}$ be the (random) consumptions of resource $k$  during the previous $t^*-1$ rounds. For each $t<t^*, j \in J$ and $e \in E_{j}$, let
$X_{j,t}$ indicate if $j$ arrives at $t$,  $Y_{e,t}$ indicate if $e$ is sampled at $t$, and $Z_{e}$ indicate if $e$ is present when probed. Thus, we have
\begin{align}
\E[U_{k,t}]& \le \E\Big[\sum_{t<t^*} \sum_{j \in J} \sum_{e \in E_{j} } X_{j,t} \cdot  Y_{e,t} \cdot Z_e\Big] 
=\sum_{t<t^*}\sum_{j \in J} \sum_{ e\in E_{j,k}}   (r_j/T)\cdot (\gam x^*_e p_e/ r_j)  \\
&= \sum_{e \in E}x^*_e p_e a_{e,k} \sum_{t<t^*} (\gam/T)  \le B_k \cdot \gam \cdot (t^*-1)/T
 \label{ineq:nadap-2}
\end{align}
Now we analyze the probability that $f^*$ is safe at $t^*$.
\begin{align}
\beta_{e^*,t^*}=\Pr\Big[  \bigwedge_{k \in \cS_{e^*}} \big(U_{k,t^*} \le B_k-1 \big)\Big] 
\ge 1- \sum_{k \in \cS_{e^*}} \Pr[U_{k,t^*} \ge B_k] \ge 1- \sum_{k \in \cS_{e^*}} \frac{E[U_{k,t^*}]}{B_k}  \ge  1- \frac{\gam  \Del (t^*-1)}{T}\label{ineq:nadap-3}
\end{align}

\end{proof}




%Due to the space limit, we present the proof of Lemma~\ref{lem:nadap-1} only for the special case when all $c_i=1$ (actually we can show this is the worst case in terms of competitive ratios). We defer a more detailed proof to the full version. 


% Consider a given $t^* \le T$ and a given assignment $f^*=(j^*,S^*)$ with $S^* \in \Lam_{j^*}$. Recall that $\SF_{f^*,t^*}$ is the event that $f^*$ is safe at $t^*$. For each $t<t^*$, let $H_{f^*,t}$ be the event that none of offline agents in $S^*$ is included in any assignment sampled at $t$. Thus, we see that $f^*$ is safe at $t^*$ iff $H_{f^*, t}$ occurs for all $t<t^*$ since all offline agents have a unit capacity. Therefore, $\SF_{f^*,t^*} =(\wedge_{t<t^*} H_{f^*,t})$. 
% Observe that $\neg H_{f^*,t}$ means at least one $j$ arrives at $t$ and an assignment $f \in \Lam_{j}$ gets sampled with $f \in \cup_{i \in S^*} \Sig_{ij}$. Thus, we have 
% $$\Pr[ H_{f^*,t}]=1-\sum_{j \in J} p_{j,t}\sum_{f \in \cup_{i \in S^*}\Sigma_{ij}} \frac{\gam \cdot(\alp_1 x^*_{f,t}+\alp_2 y^*_{f,t})}{p_{j,t}}=1-
% \sum_{j \in J}\sum_{f \in \cup_{i \in S^*} \Sigma_{ij}} \gam \Big(\alp_1 x^*_{f,t}+\alp_2 y^*_{f,t}\Big) \doteq 1-\kappa_t$$
% 
%Thus, we have 
%\begin{align}
%\Pr[\SF_{f^*,t^*}] =\Pr[\wedge_{t<t^*} H_{f^*,t}]=\prod_{t<t^*} \Pr[H_{f^*,t}]
%= \prod_{t<t^*}(1-\kappa_t) \label{ineq:nadap-1}
%\end{align}
%
%
%Here are two important observations. 
%\begin{align}
%\textbf{(Fact 1)}~~ \kappa_t
%\le \sum_{j \in J} \sum_{f\in \Lam_j} \gam \Big(\alp_1 x^*_{f,t}+\alp_2 y^*_{f,t}\Big) \le \sum_{j \in J} \gam \Big(\alp_1 p_{j,t}+ \alp_2 p_{j,t}\Big)
%  \le \gam(\alp_1 +\alp_2) \le \gam, ~~\forall t  \label{ineq:nadap-2}
%\end{align}
%The second inequality in \eqref{ineq:nadap-2} is due to Constraint~\eqref{cons:j} in \LP-\eqref{obj-1} and \LP-\eqref{obj-2}. 
%
%
%\begin{align}\label{eqn:nadap-2}
%\textbf{(Fact 2)}~~ &\sum_{t<t^*} \kappa_t 
%\le \sum_{t<t^*} \sum_{j \in J}\sum_{i \in S^*} \sum_{f\in \Sig_{ij}} \gam\Big(\alp_1 x^*_{f,t}+\alp_2 y^*_{f,t} \Big)\\
% & = \gam \sum_{i \in S^*} \left( \sum_{t<t^*} \sum_{j \in J} \sum_{f\in \Sig_{ij}}  \Big(\alp_1 x^*_{f,t}+\alp_2 y^*_{f,t} \Big)\right)
%  \le \gam \sum_{i \in S^*}  \Big(\alp_1 c_i+\alp_2 c_i \Big) \le 
%   \gam \cdot \Del \label{ineq:nadap-3}
%\end{align}
%The first inequality in \eqref{ineq:nadap-3} is due to Constraint~\eqref{cons:i} in \LP-\eqref{obj-1} and \eqref{obj-2}; the second  inequality in \eqref{ineq:nadap-3} is due to $\alp_1+\alp_2 \le 1$, all $c_i=1$, and $|S^*| \le \Del$. Applying \textbf{(Fact 1)} and \textbf{(Fact 2)} to Equality~\eqref{ineq:nadap-1}, we claim that $\Pr[\SF_{f^*,t^*}] \ge  (1-\gam)^\Del$.

%We conduct an edge by edge analysis. We can show that each assignment $f$ will be sampled and safe at $t$ with probability at least $\gam \Big(\alp_1 x_{f,t}^*+\alp_2 y_{f,t}^*\Big) (1-\gam)^\Del$. Then choose $\gam=1/(\Del+1)$, we get our claim.



\xhdr{Proof of Theorem~\ref{thm:main-2}}.
\begin{proof}
Consider a given assignment $e=(i,j)$. Let $M_{e}$ be the random number of times that $e$ is matched by $\nadap(\gam)$. For each $t \in [T]$, let $X_{t}$ indicate if $j$ arrives at $t$, $Y_{t}$ indicate if $e$ is sampled at $t$, and $Z_t$ indicate if $e$ is present when probed at $t$. Thus, we have
\begin{align}
\E[M_{e}] &=\sum_{t=1}^T \E[X_t \cdot Y_ t \cdot \SF_{e,t}\cdot Z_{t}] \ge \sum_{t=1}^T (r_j/T) \cdot  \big( \gam x_e^*/r_j \big)\cdot \Big(1- \frac{\gam  \Del (t-1)}{T}\Big) \cdot p_e
  \\
&\ge \gam x_e^*p_e \sum_{t=1}^T \frac{1}{T}\Big(1- \frac{\gam  \Del (t-1)}{T}\Big) \ge x_e^* p_e \cdot \gam \cdot \Big(1-\frac{\gam \Del}{2}\Big).
\end{align}

Thus, by setting $\gam=1/\Del$, we have $\E[M_{e}] \ge  x_e^* p_e /(2 \Del)$. By the linearity of expectation, we claim that $\alg(\gam)$ achieves competitive ratios at least $1/(2 \Del)$. 
\end{proof}

%Thus, we have $\E[X_{f^*}] \ge \alp_\ell x_{f^*}^{(\ell)} \frac{1-\sfe^{-\Del}}{\Del}$ for each $\ell\in\{1,2\}$. By the linearity of expectation, we claim that $\alg(\bsm{\alp})$ achieves a ratio at least $\alp_1\frac{1-\sfe^{-\Del}}{\Del}$ and $\alp_2\frac{1-\sfe^{-\Del}}{\Del}$ for the system efficiency and individual diversity, respectively. 







==> 6-hard.tex <==

\section{Hardness Results}
%In this section we prove the second part of Theorem~\ref{thm:main-1}.

\begin{theorem}
No algorithm can achieve a competitive ratio better than  $\big(1-\sfe^{-(\Del-1+1/\Del)}\big)/(\Del-1+1/\Del)$ with respect to the canonical benchmark \LP~\eqref{obj-1}
\end{theorem}

\begin{example}\label{exam}
Consider the projective plane $\cH=(\cV, \cE)$ of order $\Del-1$~\cite{chan2012linear}. $\cH$ is a hypergraph such that (1) $\cH$ is $\Del$-uniform, $\Del$-regular and intersecting; (2) $|\cV|=|\cE|=D \doteq \Del^2-\Del+1$, (3) the natural canonical LP on $\cH$ has an optimal value of $\Del^2-\Del+1$. Now based on $\cH$, we construct an instance of \mb as follows.

Let $G=(I,J,E)$ be a star graph with $|I|=1$, $|J|=|E|=n=T$, and $r_j=1$ for all $j \in J$. Set $K=D$, where each offline resource corresponds to one hypervertex. Set $B_k=1$ for all $k$. The set of edges $E$ has $T/D$  identical bundles and each bundle can be viewed as a copy of $\cE$. Let $\cB$ be a given bundle and every $e \in \cB$ corresponds a hyperedge $e \in \cE$ such that (1) with probability $p=(\Del-1+1/\Del)/T$, $W_e=1$ and $\cA_e=\bfa_e$, where  $\bfa_e \in \{0,1\}^D$ is the canonical vector of $e$; (2) with probability $1-p$, $W_e=0$ and $\cA_e=\bz$, where $\bz$ is the zero vector of dimension $D$. Thus, we see that every edge $e$ has a support of size $\Del$, \ie the number of non-zero entries in $\bfa_e$.
 \end{example}

%$\cA_e=\bfa_e$ with probability $p$ and $\bz$ otherwise, where  $\bfa_e \in \{0,1\}^D$ is the canonical vector of $f$. Thus, each edge $e$ has a sparsity of $\Del$. Set $p=(\Del-1+1/\Del)/T$.


\begin{lemma}
 \LP-\eqref{obj-1} has an optimal value at least $\Del-1+1/\Del$ on Example~\ref{exam}.
\end{lemma}


\begin{proof}
Let $\OPT$ be the optimal value of  \LP-\eqref{obj-1} on Example~\ref{exam}.
Consider a given unit bungle $\cB$ and for each $e \in \cB$, let $y_e$ be the sum of $x_e$ over $T/D$ copies. Consider such a solution that $x_e=1$, $y_e=T/D$ for all $e \in \cB$. We show $\{x_e\}$ is feasible to  \LP-\eqref{obj-1}. First, $\{x_e\}$ is feasible to Constraint~\eqref{cons:j}. Second,  $\{x_e\}$ is feasible to Constraint~\eqref{cons:i}, since for each $k$,  
$$\sum_{e \in E: a_{e,k}=1} x_e \E[A_{e,k}]=\sum_{e \in \cB: a_{e,k}=1} y_e \cdot p =\Del \cdot (T/D) \cdot p=1.$$

Thus, \LP-\eqref{obj-1} has an optimal value at least $\sum_{e \in \cB} y_e p= D \cdot (T/D) \cdot p=\Del-1+1/\Del$.
\end{proof}

\xhdr{Proof of the second part of Theorem~\ref{thm:main-1}}. 
%Now we start to prove the second part of Theorem~\ref{thm:main-1}.
\begin{proof}
Consider Example~\ref{exam}. Note that all the $T$ edges are intersecting with each other. We see that for any online algorithm $\ALG$, its performance should be no larger than $1-(1-p)^T=1-\sfe^{-(\Del-1+1/\Del)}$. Thus, we claim that the resultant online ratio should be no larger than $\Big(1-\sfe^{-(\Del-1+1/\Del)}\Big)/(\Del-1+1/\Del)$.
\end{proof}



%From Constraint~\eqref{cons:j}, we see $y_e \le T/D$ since each $x_e \le 1$. From  Constraint~\eqref{cons:i}, we see $\sum_{e: a_{e,k}=1} y_e \le 1/p$ for all $k$. Thus, 
%$$\sum_{k \in [K]} \sum_{e: a_{e,k}=1} y_e =\Del \sum_{e \in \cB} y_e \le K/p \implies
%\sum_{e \in \cB} y_e \le K/(p\Del) \implies \sum_{e \in \cB} y_ep_e \le K/\Del=\Del-1+1/\Del,$$
%which implies $\OPT \le \Del-1+1/\Del$. 
%
%Consider such a solution $y_e=T/D$






%are reduced to $x_e \le 1$. For each given edge $e$, let $y_e$ be the sum of $x_e$ over $T/D$ copies. 





  


%For each given hypervertex $v \in \cV$, we create a resource $k$ and thus we have $K=\Del^2-\Del+1$ total resources. Set $B_k=1$ for all $k \in [K]$. For each hyperedge $f \in \cE$, we create an edge $e$ with $\ba_{e}$ being the canonical vector of $f$. Thus, we have $\Del^2-\Del+1$ distinct edges called a bundle. Create $T/(\Del^2-\Del+1)$ identical copies of bundle and we have in total 
 

%(\ie $a_{k,e}=1$ iff $f \ni v$ where $v$ correpson) 



%Let $K=\Del^2-\Del+1$ and each resource corresponds to a hypervertex in $\cH$.  

   






